Island Cosmology

If the observed dark energy is a cosmological constant, the canonical state of the universe is de Sitter spacetime. In such a spacetime, quantum fluctuations that violate the null energy condition will create islands of matter that, if large enough, may resemble our observable universe. Phenomenological approaches to calculating density fluctuations yield a scale invariant spectrum with suitable amplitude. With time, the island of matter that is our observable universe, re-enters the cosmological constant sea.

==> svind.ist.tex <==
 delim_0 "\\idxquad "delim_1 "\\idxquad "delim_2 "\\idxquad "delim_n ",\\,"
